Robust Interference Management for SISO Systems with Multiple Over-the-Air Computations

In this paper, we consider the over-the-air computation of sums. Specifically, we wish to compute $M\geq 2$ sums $s_m=\sum_{k\in\mathcal{D}m}x_k$ over a shared complex-valued MAC at once with minimal mean-squared error ($\mathsf{MSE}$). Finding appropriate Tx-Rx scaling factors balance between a low error in the computation of $s_n$ and the interference induced by it in the computation of other sums $s_m$, $m\neq n$. In this paper, we are interested in designing an optimal Tx-Rx scaling policy that minimizes the mean-squared error $\max_{m\in[1:M]}\mathsf{MSE}_m$ subject to a Tx power constraint with maximum power $P$. We show that an optimal design of the Tx-Rx scaling policy $\left(\bar{\mathbf{a}},\bar{\mathbf{b}}\right)$ involves optimizing (a) their phases and (b) their absolute values in order to (i) decompose the computation of $M$ sums into, respectively, $M_R$ and $M_I$ ($M=M_R+M_I$) calculations over real and imaginary part of the Rx signal and (ii) to minimize the computation over each part -- real and imaginary -- individually. The primary focus of this paper is on (b). We derive conditions (i) on the feasibility of the optimization problem and (ii) on the Tx-Rx scaling policy of a local minimum for $M_w=2$ computations over the real ($w=R$) or the imaginary ($w=I$) part. Extensive simulations over a single Rx chain for $M_w=2$ show that the level of interference in terms of $\Delta D=|\mathcal{D}_2|-|\mathcal{D}_1|$ plays an important role on the ergodic worst-case $\mathsf{MSE}$. At very high $\mathsf{SNR}$, typically only the sensor with the weakest channel transmits with full power while all remaining sensors transmit with less to limit the interference. Interestingly, we observe that due to residual interference, the ergodic worst-case $\mathsf{MSE}$ is not vanishing; rather, it converges to $\frac{|\mathcal{D}_1||\mathcal{D}_2|}{K}$ as $\mathsf{SNR}\rightarrow\infty$.

==> Feas_Anal_SNR_Impact_Plot.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.20000,0.60000,0.50000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=3.61in,
height=3.566in,
at={(0.605in,0.481in)},
scale only axis,
bar shift auto,
xmin=0.514285714285714,
xmax=3.48571428571429,
xtick={1,2,3},
xticklabels={{\footnotesize $\left(|\mathcal{D}_1|,|\mathcal{D}_2|\right)=(1,29)$},{\footnotesize $\left(|\mathcal{D}_1|,|\mathcal{D}_2|\right)=(3,27)$},{\footnotesize $\left(|\mathcal{D}_1|,|\mathcal{D}_2|\right)=(5,25)$}},
ymin=0,
ymax=2700,
ylabel style={font=\color{white!15!black}},
ylabel={\footnotesize Frequency},
axis background/.style={fill=white},
% legend style={legend cell align=left, align=left, draw=white!15!black},
legend pos=outer north east,
]
\addplot[ybar, bar width=10, fill=red, draw=black, area legend] table[row sep=crcr] {%
1	2500\\
2	1689\\
3	49\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0.514285714285714	0\\
3.48571428571429	0\\
};
\addlegendentry{infeasible}

\addplot[ybar, bar width=10, fill=mycolor1, draw=black, area legend] table[row sep=crcr] {%
1	0\\
2	811\\
3	2451\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0.514285714285714	0\\
3.48571428571429	0\\
};
\addlegendentry{feasible}

\node[above, align=center]
at (axis cs:0.857,2500) {2500};
\node[above, align=center]
at (axis cs:1.857,1689) {1689};
\node[above, align=center]
at (axis cs:2.857,49) {49};
\node[above, align=center]
at (axis cs:1.143,0) {0};
\node[above, align=center]
at (axis cs:2.143,811) {811};
\node[above, align=center]
at (axis cs:3.143,2451) {2451};
\end{axis}
\end{tikzpicture}%

==> tikzlibrarysignalflowarrows.code.tex <==
% pgf/tikz library
% for signal flow diagrams
%
% Author: Dr. Karlheinz Ochs, Ruhr-University of Bochum, Germany
% Version: 0.1
% Date: 2007/01/05


% Styles for real and complex signal tips.
\newcommand{\pgfarrowsextend}[1]{%
  \pgfsetcolor{\pathdrawcolor}%
  \@tempdima=#1\pgflinewidth%
  \pgfarrowsleftextend{-2\@tempdima}
  \pgfarrowsrightextend{2\@tempdima}
}
\newcommand{\pgfarrowsarrowtip}[1]{%
  \pgfsetcolor{\pathdrawcolor}%
  \@tempdima=#1\pgflinewidth%
  \pgfpathmoveto{\pgfpoint{2\@tempdima}{0pt}}
  \pgfpathlineto{\pgfpoint{-\@tempdima}{\@tempdima}}
  \pgfpathlineto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{-\@tempdima}{-\@tempdima}}
  \pgfusepathqfill
}
\pgfarrowsdeclare{real tip}{real tip}{\pgfarrowsextend{3}}{\pgfarrowsarrowtip{3}}
\pgfarrowsdeclarereversed{real tip reversed}{real tip reversed}{real tip}{real tip}
\pgfarrowsdeclare{complex tip}{complex tip}{\pgfarrowsextend{1}}{\pgfarrowsarrowtip{1}}
\pgfarrowsdeclarereversed{complex tip reversed}{complex tip reversed}{complex tip}{complex tip}


\endinput


==> tikzlibrarysignalflowblocks.code.tex <==
% pgf/tikz library
% for signal flow diagrams
%
% Author: Dr. Karlheinz Ochs, Ruhr-University of Bochum, Germany
% Version: 0.1
% Date: 2007/01/05

% Known bugs: - Anchors of source shape are not precisely positioned.
%             - Anchor border of source shape is a rectangle.
%             - The bounding box of standard text label is ignored.


%
% Styles for nodes, terminals, and operators.
%
% - building blocks
\tikzstyle{block color}%
   = [draw=\blockdrawcolor,
      fill=\blockfillcolor]
\tikzstyle{block style}%
   = [block color,
      line width=\blocklinewidth,
      text centered]
\tikzstyle{block}%
   = [rectangle,
      block style,
      minimum width=\blockwidth,
      minimum height=\blockheight,
      text width=\blocktextwidth]
\tikzstyle{filter}%
   = [rectangle,
      block style,
      minimum width=\filterwidth,
      minimum height=\filterheight,
      text width=\filtertextwidth]
\tikzstyle{source}%
   = [source shape,
      operator style]
\tikzstyle{serial parallel converter}%
   = [serial parallel converter shape,
      block style,
      minimum width=10mm,
      minimum height=20mm,
      inner sep=2mm]
\tikzstyle{parallel serial converter}%
   = [parallel serial converter shape,
      block style,
      minimum width=10mm,
      minimum height=20mm,
      inner sep=2mm]
\tikzstyle{symbol mapper}%
   = [symbol mapper shape,
      block style,
      text centered,
      minimum size=20mm,
      text width=18mm]
\tikzstyle{inverse symbol mapper}%
   = [inverse symbol mapper shape,
      block style,
      text centered,
      minimum size=20mm,
      text width=18mm]


%
% Shape of a source.
%
\newbox\pgfnodeparttextbox
\pgfdeclareshape{source shape}
{
  \savedanchor\westpoint{
    \pgf@x=\wd\pgfnodeparttextbox%
    \advance\pgf@x by\pgfshapeouterxsep%
    \pgf@y=.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by-.5\dp\pgfnodeparttextbox%
  }
  \saveddimen\radius{
    \setlength\pgf@x{\pgfshapeminwidth}
  }
  \anchor{west}{\westpoint}
  \anchor{north west}{
    \pgf@process{\westpoint}
    \advance\pgf@y by\radius
  }
  \anchor{north}{%
    \pgf@process{\westpoint}
    \pgf@xa=\radius\advance\pgf@x by+0.5\pgf@xa
    \pgf@ya=\radius\advance\pgf@y by+0.866025\pgf@ya
  }
  \anchor{north east}{%
    \pgf@process{\westpoint}
    \pgf@xa=\radius\advance\pgf@x by+0.866025\pgf@xa
    \pgf@ya=\radius\advance\pgf@y by+0.5\pgf@ya
  }
  \anchor{east}{
    \pgf@process{\westpoint}
    \advance\pgf@x by\radius
    \advance\pgf@x by0.5\pgflinewidth
  }
  \anchor{south east}{%
    \pgf@process{\westpoint}
    \pgf@xa=\radius\advance\pgf@x by+0.866025\pgf@xa
    \pgf@ya=\radius\advance\pgf@y by-0.5\pgf@ya
  }
  \anchor{south}{%
    \pgf@process{\westpoint}
    \pgf@xa=\radius\advance\pgf@x by+0.5\pgf@xa
    \pgf@ya=\radius\advance\pgf@y by-0.866025\pgf@ya
  }
  \anchor{south west}{
    \pgf@process{\westpoint}
    \advance\pgf@y by-\radius
  }
  \anchor{center}{
    \pgf@process{\westpoint}
    \pgf@xa=\radius\advance\pgf@x by+0.5\pgf@xa
  }
  % node part
  \nodeparts{text}
  \anchor{text}{
    \pgf@process{\westpoint}
    \pgf@xa=\radius
    \advance\pgf@y by-.5\ht\pgfnodeparttextbox%
    \advance\pgf@x by-\wd\pgfnodeparttextbox%
    \advance\pgf@x by-0.5mm
  }
  \anchorborder{%
    \pgf@xb=\pgf@x% xb/yb is target
    \pgf@yb=\pgf@y%
    % southwest
    \westpoint\advance\pgf@y by-\radius
    \pgf@xa=\pgf@x% xa/ya is se
    \pgf@ya=\pgf@y%
    % northeast
    \westpoint\advance\pgf@x by\radius\advance\pgf@y by\radius%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgf@xc=.5\pgf@x% x/y is half width/height
    \pgf@yc=.5\pgf@y%
    \advance\pgf@xa by\pgf@xc% xa/ya becomes center
    \advance\pgf@ya by\pgf@yc%
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderrectangle
      {\noexpand\pgfpoint{\the\pgf@xb}{\the\pgf@yb}}
      {\noexpand\pgfpoint{\the\pgf@xc}{\the\pgf@yc}}%
    }%
    \pgf@process{\pgf@marshal}%
    \advance\pgf@x by\pgf@xa%
    \advance\pgf@y by\pgf@ya%
  }
  % Background path
  \backgroundpath{
  {\pgftransformreset{\pgfnodeparttextbox}}
    \westpoint \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \advance\pgf@y by\radius
    \pgfmoveto{\pgfpoint{\pgf@x}{\pgf@y}}
    \pgfpatharc{90}{-90}{\radius}
    \pgfclosepath
 }
}


%
% Shape of a serial to parallel converter.
%
\newbox\pgfnodepartSbox
\newbox\pgfnodepartPbox
\pgfdeclareshape{serial parallel converter shape}
{
  % inherit from rectangle
  \inheritsavedanchors[from=rectangle]
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{south east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchorborder[from=rectangle]
  \inheritanchorborder[from=rectangle]
  \inheritbackgroundpath[from=rectangle]
  % terminal anchors
  \anchor{in}{%
    \northeast
    \pgf@ya=0.5\pgf@y
    \southwest
    \pgf@y=0.5\pgf@y
    \advance\pgf@y by+\pgf@ya%
  }
  \anchor{out1}{
    \southwest
    \pgf@ya=0.9\pgf@y
    \northeast
    \pgf@y=0.1\pgf@y
    \advance\pgf@y by\pgf@ya%
  }
  \anchor{out2}{
    \southwest
    \pgf@ya=0.7\pgf@y
    \northeast
    \pgf@y=0.3\pgf@y
    \advance\pgf@y by\pgf@ya%
  }
  \anchor{outl}{
    \southwest
    \pgf@ya=0.1\pgf@y
    \northeast
    \pgf@y=0.9\pgf@y
    \advance\pgf@y by\pgf@ya%
  }
  \anchor{dots}{
    \southwest
    \pgf@ya=0.4\pgf@y
    \northeast
    \pgf@y=0.6\pgf@y
    \advance\pgf@y by\pgf@ya%
    \setlength{\pgf@xa}{\xspace}
    \advance\pgf@x by.5\pgf@xa%
  }
  % node parts
  \nodeparts{S,P}
  \anchor{S}{
    \southwest
    \pgf@xa=\pgf@x
    \northeast
    \pgf@x=\pgf@xa
    \advance\pgf@y by-\ht\pgfnodepartSbox%
    \advance\pgf@y by-.5\dp\pgfnodepartSbox%
    \advance\pgf@x by+\pgfshapeinnerxsep%
    \advance\pgf@y by-\pgfshapeinnerysep%
  }
  \anchor{P}{
    \northeast
    \pgf@xa=\pgf@x
    \southwest
    \pgf@x=\pgf@xa
    \advance\pgf@x by-\wd\pgfnodepartPbox%
    \advance\pgf@x by-\pgfshapeinnerxsep%
    \advance\pgf@y by+\pgfshapeinnerysep%
  }
  % diagonal line S/P
  \foregroundpath{%
    \pgfpathmoveto{\pgfpointadd{\southwest}{\pgfpoint{\pgfshapeouterxsep}{\pgfshapeouterysep}}}
    \pgfpathlineto{\pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfshapeouterxsep}{\pgfshapeouterysep}}}}
  }
}

%
% Shape of a parallel to serial converter.
%
\newbox\pgfnodepartSbox
\newbox\pgfnodepartPbox
\pgfdeclareshape{parallel serial converter shape}
{
  % inherit from rectangle
  \inheritsavedanchors[from=rectangle]
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{south east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchorborder[from=rectangle]
  \inheritanchorborder[from=rectangle]
  \inheritbackgroundpath[from=rectangle]
  % terminal anchors
  \anchor{out}{%
    \southwest
    \pgf@ya=0.5\pgf@y
    \northeast
    \pgf@y=0.5\pgf@y
    \advance\pgf@y by+\pgf@ya%
  }
  \anchor{in1}{
    \northeast
    \pgf@ya=0.1\pgf@y
    \southwest
    \pgf@y=0.9\pgf@y
    \advance\pgf@y by\pgf@ya%
  }
  \anchor{in2}{
    \northeast
    \pgf@ya=0.3\pgf@y
    \southwest
    \pgf@y=0.7\pgf@y
    \advance\pgf@y by\pgf@ya%
  }
  \anchor{inl}{
    \northeast
    \pgf@ya=0.9\pgf@y
    \southwest
    \pgf@y=0.1\pgf@y
    \advance\pgf@y by\pgf@ya%
  }
  \anchor{dots}{
    \northeast
    \pgf@ya=0.6\pgf@y
    \southwest
    \pgf@y=0.4\pgf@y
    \advance\pgf@y by\pgf@ya%
    \setlength{\pgf@xa}{\xspace}
    \advance\pgf@x by-.5\pgf@xa%
  }
  % node parts
  \nodeparts{P,S}
  \anchor{P}{
    \southwest
    \pgf@xa=\pgf@x
    \northeast
    \pgf@x=\pgf@xa
    \advance\pgf@y by-\ht\pgfnodepartPbox%
    \advance\pgf@y by-.5\dp\pgfnodepartPbox%
    \advance\pgf@x by+\pgfshapeinnerxsep%
    \advance\pgf@y by-\pgfshapeinnerysep%
  }
  \anchor{S}{
    \northeast
    \pgf@xa=\pgf@x
    \southwest
    \pgf@x=\pgf@xa
    \advance\pgf@x by-\wd\pgfnodepartSbox%
    \advance\pgf@x by-\pgfshapeinnerxsep%
    \advance\pgf@y by+\pgfshapeinnerysep%
  }
  % diagonal line S/P
  \foregroundpath{%
    \pgfpathmoveto{\pgfpointadd{\southwest}{\pgfpoint{\pgfshapeouterxsep}{\pgfshapeouterysep}}}
    \pgfpathlineto{\pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfshapeouterxsep}{\pgfshapeouterysep}}}}
  }
}


%
% Shape of a symbol mapper.
%
\pgfdeclareshape{symbol mapper shape}
{
  % rectangle anchors
  \inheritsavedanchors[from=rectangle]
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{south east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchorborder[from=rectangle]
  % terminal anchors
  \anchor{out}{%
    \southwest
    \pgf@ya=0.5\pgf@y
    \northeast
    \pgf@y=0.5\pgf@y
    \advance\pgf@y by+\pgf@ya%
  }
  \anchor{in1}{
    \northeast
    \pgf@ya=0.1\pgf@y
    \southwest
    \pgf@y=0.9\pgf@y
    \advance\pgf@y by\pgf@ya%
  }
  \anchor{in2}{
    \northeast
    \pgf@ya=0.3\pgf@y
    \southwest
    \pgf@y=0.7\pgf@y
    \advance\pgf@y by\pgf@ya%
  }
  \anchor{dots}{
    \northeast
    \pgf@ya=0.6\pgf@y
    \southwest
    \pgf@y=0.4\pgf@y
    \advance\pgf@y by\pgf@ya%
    \setlength{\pgf@xa}{\xspace}
    \advance\pgf@x by-.5\pgf@xa%
  }
  \anchor{inl}{
    \northeast
    \pgf@ya=0.9\pgf@y
    \southwest
    \pgf@y=0.1\pgf@y
    \advance\pgf@y by\pgf@ya%
  }
  % rectangle shaped frame
  \backgroundpath{
    \pgfpathrectanglecorners
    {\pgfpointadd{\southwest}{\pgfpoint{\pgfshapeouterxsep}{\pgfshapeouterysep}}}
    {\pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfshapeouterxsep}{\pgfshapeouterysep}}}}
  }

  \inheritbackgroundpath[from=rectangle]
}


%
% Shape of an inverse symbol mapper.
%
\pgfdeclareshape{inverse symbol mapper shape}
{
  % rectangle anchors
  \inheritsavedanchors[from=rectangle]
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{south east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchorborder[from=rectangle]
  % terminal anchors
  \anchor{in}{%
    \northeast
    \pgf@ya=0.5\pgf@y
    \southwest
    \pgf@y=0.5\pgf@y
    \advance\pgf@y by+\pgf@ya%
  }
  \anchor{out1}{
    \southwest
    \pgf@ya=0.9\pgf@y
    \northeast
    \pgf@y=0.1\pgf@y
    \advance\pgf@y by\pgf@ya%
  }
  \anchor{out2}{
    \southwest
    \pgf@ya=0.7\pgf@y
    \northeast
    \pgf@y=0.3\pgf@y
    \advance\pgf@y by\pgf@ya%
  }
  \anchor{outl}{
    \southwest
    \pgf@ya=0.1\pgf@y
    \northeast
    \pgf@y=0.9\pgf@y
    \advance\pgf@y by\pgf@ya%
  }
  \anchor{dots}{
    \southwest
    \pgf@ya=0.4\pgf@y
    \northeast
    \pgf@y=0.6\pgf@y
    \advance\pgf@y by\pgf@ya%
    \setlength{\pgf@xa}{\xspace}
    \advance\pgf@x by.5\pgf@xa%
  }
  % rectangle shaped frame
  \backgroundpath{
    \pgfpathrectanglecorners
    {\pgfpointadd{\southwest}{\pgfpoint{\pgfshapeouterxsep}{\pgfshapeouterysep}}}
    {\pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfshapeouterxsep}{\pgfshapeouterysep}}}}
  }

  \inheritbackgroundpath[from=rectangle]
}

\endinput


==> tikzlibrarysignalflowdiagram.code.tex <==
% pgf/tikz library
% for signal flow diagrams
%
% Author: Dr. Karlheinz Ochs, Ruhr-University of Bochum, Germany
% Version: 0.1
% Date: 2007/01/05

%
% Extended general shape options, cf. tikz.code.tex
%
% #1 = source node
% Remark: The node distance is used
%         for the distance between the borders of two nodes
\tikzoption{below from}{\tikz@from{#1}{1}{-90}{south}{north}}%
\tikzoption{right from}{\tikz@from{#1}{1}{0}{east}{west}}%
\tikzoption{above from}{\tikz@from{#1}{1}{90}{north}{south}}%
\tikzoption{left from}{\tikz@from{#1}{1}{180}{west}{east}}%
\tikzoption{below left from}{\tikz@from{#1}{1.414214}{-135}{south west}{north east}}%
\tikzoption{below right from}{\tikz@from{#1}{1.414214}{-45}{south east}{north west}}%
\tikzoption{above right from}{\tikz@from{#1}{1.414214}{45}{north east}{south west}}%
\tikzoption{above left from}{\tikz@from{#1}{1.414214}{135}{north west}{south east}}%
\def\tikz@from#1#2#3#4#5{%
  \def\tikz@anchor{#5}%
  \let\tikz@do@auto@anchor=\relax%
  \tikz@addtransform{\pgftransformshift{\pgfpointscale{#2}{\pgfpointpolar{#3}{\tikz@node@distance}}}}%
  \def\tikz@node@at{\pgfpointanchor{#1}{#4}}}


%
% Styles for real and complex signal paths.
%
\tikzstyle{dotted path}
   = [loosely dotted,
      shorten >= 2mm,
      shorten <= 2mm]
\tikzstyle{r}
   = [line width=\pathlinewidth,
      >= real tip,
      draw]
\tikzstyle{r>}
   = [r,->]
\tikzstyle{<r}
   = [r,<-]
\tikzstyle{r.}
   = [r,dotted path]
\tikzstyle{c}
   = [line width=\pathlinewidth,
      double=\pathfillcolor,
      double distance=\pathlinewidth,
      >= complex tip,
      draw,shorten <=-\pathlineextend]
\tikzstyle{c>}
   = [c,->]
\tikzstyle{<c}
   = [c,<-]
\tikzstyle{c.}
   = [c,dotted path]


\endinput


==> tikzlibrarysignalflowoperators.code.tex <==
% pgf/tikz library
% for signal flow diagrams
%
% Author: Dr. Karlheinz Ochs, Ruhr-University of Bochum, Germany
% Version: 0.1
% Date: 2007/01/05


%
% Styles for nodes, terminals, and operators.
%
% - nodes and terminals
\tikzstyle{node style}%
   = [draw=\pathdrawcolor,
      fill=\pathdrawcolor,
      minimum size=\nodesize]
\tikzstyle{terminal style}%
   = [draw=\pathdrawcolor,
      fill=\pathfillcolor,
      line width=\pathlinewidth,
      minimum size=\terminalsize]
\tikzstyle{node}%
   = [node shape,
      node style]
\tikzstyle{input}%
   = [input terminal shape,
      terminal style]
\tikzstyle{output}%
   = [output terminal shape,
      terminal style]
% - operators
\tikzstyle{operator color}%
   = [draw=\operatordrawcolor,
      fill=\operatorfillcolor]
\tikzstyle{operator style}%
   = [operator color,
      line width=\operatorlinewidth,
      minimum size=\operatorsize]
\tikzstyle{multiplier}%
   = [multiplier shape,
      operator style]
\tikzstyle{modulator}%
   = [modulator shape,
      operator style]
\tikzstyle{adder}%
   = [adder shape,
      operator style]
\tikzstyle{delay}%
   = [rectangle,
      operator style,
      minimum size=\delaysize]


%
% Circular shapes of operator symbols.
%
% #1 = additional inner symbol
\newcommand{\circularshape}[1]{%
  \savedanchor\centerpoint{\pgfpointorigin}
  % radius is half of maximum of \pgfshapeminwidth and \pgfshapeminheight
  \saveddimen\radius{%
    \setlength{\pgf@xa}{\pgfshapeminwidth}
    \setlength{\pgf@ya}{\pgfshapeminheight}
    \ifdim\pgf@xa>\pgf@ya
      \pgf@x=.5\pgf@xa
    \else
      \pgf@x=.5\pgf@ya
    \fi
  }
  \inheritanchor[from=circle]{center}
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{south east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  % circular shaped frame
  \inheritbackgroundpath[from=circle]
  % additional inner symbol
  \foregroundpath{
    \centerpoint%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \@tempdima=\radius%
    #1
  }
  % no text
  \nodeparts{}
}


%
% Anchors for default text box, see below.
%
\newcommand{\stdaboveanchor}{%
  \anchor{text}{%
    \centerpoint
    \advance\pgf@x by-0.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by\radius
    \advance\pgf@y by+0.5mm
  }
}
\newcommand{\stdrightanchor}{%
  \anchor{text}{%
    \centerpoint
    \advance\pgf@x by\radius
    \advance\pgf@x by+0.5mm
    \advance\pgf@y by-0.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by+0.5\dp\pgfnodeparttextbox%
  }
}
\newcommand{\stdbelowanchor}{%
  \anchor{text}{%
    \centerpoint
    \advance\pgf@x by-0.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by-\ht\pgfnodeparttextbox%
    \advance\pgf@y by-\radius
    \advance\pgf@y by-0.5mm
  }
}
\newcommand{\stdleftanchor}{%
  \anchor{text}{%
    \centerpoint
    \advance\pgf@x by-\radius
    \advance\pgf@x by-\wd\pgfnodeparttextbox%
    \advance\pgf@x by-0.5mm
    \advance\pgf@y by-0.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by+0.5\dp\pgfnodeparttextbox%
  }
}


%
% Circular shapes of operator symbols with default text box.
%
% #1 = place of the default text box
\newbox\pgfnodepartabovebox
\newbox\pgfnodepartrightbox
\newbox\pgfnodepartbelowbox
\newbox\pgfnodepartleftbox
\newcommand{\labelledcircularshape}[1]{%
  % node parts
  \nodeparts{text,above,right,below,left}
  % anchors
  \savedanchor\centerpoint{\pgfpointorigin}
  % radius is half of maximum of \pgfshapeminwidth and \pgfshapeminheight
  \saveddimen\radius{%
    \setlength{\pgf@xa}{\pgfshapeminwidth}
    \setlength{\pgf@ya}{\pgfshapeminheight}
    \ifdim\pgf@xa>\pgf@ya
      \pgf@x=.5\pgf@xa
    \else
      \pgf@x=.5\pgf@ya
    \fi
  }
  \inheritanchor[from=circle]{center}
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{south east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  #1
  \anchor{above}{%
    \centerpoint
    \advance\pgf@x by-0.5\wd\pgfnodepartabovebox%
    \advance\pgf@y by\radius
    \advance\pgf@y by+0.5mm
  }
  \anchor{right}{%
    \centerpoint
    \advance\pgf@x by\radius
    \advance\pgf@x by+0.5mm
    \advance\pgf@y by-0.5\ht\pgfnodepartrightbox%
    \advance\pgf@y by+0.5\dp\pgfnodeparttextbox%
  }
  \anchor{below}{%
    \centerpoint
    \advance\pgf@x by-0.5\wd\pgfnodepartbelowbox%
    \advance\pgf@y by-\ht\pgfnodepartbelowbox%
    \advance\pgf@y by-\radius
    \advance\pgf@y by-0.5mm
  }
  \anchor{left}{%
    \centerpoint
    \advance\pgf@x by-\radius
    \advance\pgf@x by-\wd\pgfnodepartleftbox%
    \advance\pgf@x by-0.5mm
    \advance\pgf@y by-0.5\ht\pgfnodepartleftbox%
    \advance\pgf@y by+0.5\dp\pgfnodeparttextbox%
  }
  % circular shaped frame
  \inheritbackgroundpath[from=circle]
}


%
% Shape of a node.
%
\pgfdeclareshape{node shape}{\labelledcircularshape{\stdaboveanchor}}%

%
% Shape of an input terminal.
%
\pgfdeclareshape{input terminal shape}{\labelledcircularshape{\stdleftanchor}}%
%
% Shape of an output terminal.
%
\pgfdeclareshape{output terminal shape}{\labelledcircularshape{\stdrightanchor}}%
%
% Shape of a multiplier.
%
\pgfdeclareshape{multiplier shape}{\labelledcircularshape{\stdleftanchor}}%
%
% Shape of a modulator.
%
\pgfdeclareshape{modulator shape}{\circularshape{%
    \pgfpathmoveto{\pgfpointadd{\pgfpoint{\pgf@xc}{\pgf@yc}}
                  {\pgfpoint{-0.707107\@tempdima}{-0.707107\@tempdima}}}
    \pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xc}{\pgf@yc}}
                  {\pgfpoint{0.707107\@tempdima}{0.707107\@tempdima}}}
    \pgfpathmoveto{\pgfpointadd{\pgfpoint{\pgf@xc}{\pgf@yc}}
                  {\pgfpoint{0.707107\@tempdima}{-0.707107\@tempdima}}}
    \pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xc}{\pgf@yc}}
                  {\pgfpoint{-0.707107\@tempdima}{0.707107\@tempdima}}}
}}%
%
% Shape of an adder.
%
\pgfdeclareshape{adder shape}{\circularshape{%
    \pgfpathmoveto{\pgfpointadd{\pgfpoint{\pgf@xc}{\pgf@yc}}
                  {\pgfpoint{-0.5\@tempdima}{0\@tempdima}}}
    \pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xc}{\pgf@yc}}
                  {\pgfpoint{0.5\@tempdima}{0\@tempdima}}}
    \pgfpathmoveto{\pgfpointadd{\pgfpoint{\pgf@xc}{\pgf@yc}}
                  {\pgfpoint{0\@tempdima}{-0.5\@tempdima}}}
    \pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xc}{\pgf@yc}}
                  {\pgfpoint{0\@tempdima}{0.5\@tempdima}}}
}}%

\endinput

